On MPC without terminal conditions for dynamic non-holonomic robots

We consider an input-constrained differential-drive robot with actuator dynamics. For this system, we establish asymptotic stability of the origin on arbitrary compact, convex sets using Model Predictive Control (MPC) without stabilizing terminal conditions despite the presence of state constraints and actuator dynamics. We note that the problem without those two additional ingredients was essentially solved beforehand, despite the fact that the linearization is not stabilizable. We propose an approach successfully solving the task at hand by combining the theory of barriers to characterize the viability kernel and an MPC framework based on so-called cost controllability. Moreover, we present a numerical case study to derive quantitative bounds on the required length of the prediction horizon. To this end, we investigate the boundary of the viability kernel and a neighbourhood of the origin, i.e. the most interesting areas.

==> ACSD-preamble.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% ACSD %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%% Packages
\usepackage{xspace}
\usepackage{soul}
\usepackage{mathtools}
\usepackage{makecell}
\usepackage{cite}
\usepackage{nicefrac}
\usepackage{float}
\usepackage{wrapfig}
\usepackage{amsthm}

%%%% Arrows
\newcommand{\ra}{\rightarrow}
\newcommand{\rra}{\rightrightarrows}
\newcommand{\la}{\leftarrow}
\newcommand{\Ra}{\Rightarrow}
\newcommand{\La}{\Leftarrow}
\newcommand{\LRa}{\LeftRightarrow}

%%%% Theorems
%\newtheorem{dfn}{Definition}
%\newtheorem{asm}{Assumption}
%\newtheorem{fct}{Fact}
%\newtheorem*{fct*}{Fact}
%\newtheorem{prp}{Proposition}
%\newtheorem*{prp*}{Proposition}
%\newtheorem{lem}{Lemma}
%\newtheorem*{lem*}{Lemma}
%\newtheorem{thm}{Theorem}
%\newtheorem{crl}{Corollary}
%\newtheorem*{crl*}{Corollary}
%\newtheorem{rem}{Remark}
%\newtheorem*{rem*}{Remark}
%\newtheorem{exm}{Example}
%\newtheorem*{exm*}{Example}
%\newtheorem{prb}{Problem}
%\newtheorem*{prb*}{Problem}

%%%% Abbreviations
\newcommand{\ie}{\unskip, i.\,e.,\xspace}
\newcommand{\eg}{\unskip, e.\,g.,\xspace}
\newcommand{\pd}{p.\,d.\xspace}
\newcommand{\sut}{\text{s.\,t.\,}}
\newcommand{\wrt}{w.\,r.\,t.\xspace}
\newcommand{\rt}{r.\,t.\xspace}

%%%% Sets
\newcommand{\N}{\ensuremath{\mathbb{N}}}
\newcommand{\Z}{\ensuremath{\mathbb{Z}}}
\newcommand{\Q}{\ensuremath{\mathbb{Q}}}
\newcommand{\R}{\ensuremath{\mathbb{R}}}
\newcommand{\C}{\ensuremath{\mathbb{C}}}

\newcommand{\T}{\ensuremath{\mathbb{T}}}
\newcommand{\X}{\ensuremath{\mathbb{X}}}
\newcommand{\Y}{\ensuremath{\mathbb{Y}}}
\newcommand{\F}{\ensuremath{\mathbb{F}}}
\newcommand{\U}{\ensuremath{\mathbb{U}}}

\newcommand{\sm}{\ensuremath{\setminus}}

\let\oldemptyset\emptyset
\let\emptyset\varnothing

%%%% Texts
\newcommand{\diam}{\ensuremath{\text{diam}}}
\newcommand{\dom}{\ensuremath{\text{dom}}}
\newcommand{\sgn}{\ensuremath{\text{sgn}}}
\newcommand{\co}{\ensuremath{\text{co}}}
\newcommand{\cco}{\ensuremath{\overline{\text{co}}}}

%%%% Fonts
\newcommand{\bb}[1]{\textbf{#1}}
\newcommand{\ii}[1]{\textit{#1}}
\newcommand{\bs}[1]{\ensuremath{\boldsymbol{#1}}}

%%%% Symbols
\newcommand{\eps}{\ensuremath{\varepsilon}}
\newcommand*\diff{\mathop{}\!\mathrm{d}}
\newcommand{\pdiff}[2]{ \ensuremath{ \frac{\partial {#1}}{\partial {#2}} } }
\newcommand*\circled[1]{\tikz[baseline=(char.base)]{\node[shape=circle,draw,inner sep=1pt] (char) {#1};}}
\newcommand{\ball}{\ensuremath{\mathcal B}}
\newcommand{\tp}{^{\top}}			% Transpose
\newcommand{\D}{\ensuremath{\mathcal{D}}}		% Generalized derivative
\newcommand{\K}{\ensuremath{\mathcal{K}}\xspace}		% Capital kappa
\newcommand{\KL}{\ensuremath{\mathcal{KL}}\xspace}		% Kappa-ell
\newcommand{\Kinf}{\ensuremath{\mathcal{K}_{\infty}}\xspace}		% Kappa-infinity
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\arginf}{arg\,inf}
\DeclareMathOperator*{\argsup}{arg\,sup}

%%%% References
\newcommand{\reffig}[1]{Fig.\,\ref{#1}}  
%\newcommand{\refFig}[1]{Figure\, \ref{#1}} 

%%%% Wraps
\newcommand{\norm}[1]{\left\lVert#1\right\rVert}
\newcommand{\abs}[1]{\left\lvert#1\right\rvert}
\newcommand{\scal}[1]{\left\langle#1\right\rangle}

%%%% Probability
\newcommand{\PP}{\ensuremath{\mathbb{P}}}
\newcommand{\E}{\ensuremath{\mathbb{E}}}

%%%% Review
\newcommand{\red}[1]{\textcolor{red}{#1}}
\newcommand{\blue}[1]{\textcolor{blue}{#1}}
\definecolor{dgreen}{rgb}{0.0, 0.5, 0.0}
\newcommand{\green}[1]{\textcolor{dgreen}{#1}}

%%%% Miscellaneous
\newcommand{\spc}{\ensuremath{\,\,}}	% Logical formula separator

%%%% Environments
\makeatletter
\newcommand{\subalign}[1]{%
	\vcenter{%
		\Let@ \restore@math@cr \default@tag
		\baselineskip\fontdimen10 \scriptfont\tw@
		\advance\baselineskip\fontdimen12 \scriptfont\tw@
		\lineskip\thr@@\fontdimen8 \scriptfont\thr@@
		\lineskiplimit\lineskip
		\ialign{\hfil$\m@th\scriptstyle##$&$\m@th\scriptstyle{}##$\crcr
			#1\crcr
		}%
	}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
